Large Language Models as Source Planner for Personalized Knowledge-grounded Dialogue

Open-domain dialogue system usually requires different sources of knowledge to generate more informative and evidential responses. However, existing knowledge-grounded dialogue systems either focus on a single knowledge source or overlook the dependency between multiple sources of knowledge, which may result in generating inconsistent or even paradoxical responses. To incorporate multiple knowledge sources and dependencies between them, we propose SAFARI, a novel framework that leverages the exceptional capabilities of large language models (LLMs) in planning, understanding, and incorporating under both supervised and unsupervised settings. Specifically, SAFARI decouples the knowledge grounding into multiple sources and response generation, which allows easy extension to various knowledge sources including the possibility of not using any sources. To study the problem, we construct a personalized knowledge-grounded dialogue dataset \textit{\textbf{K}nowledge \textbf{B}ehind \textbf{P}ersona}~(\textbf{KBP}), which is the first to consider the dependency between persona and implicit knowledge. Experimental results on the KBP dataset demonstrate that the SAFARI framework can effectively produce persona-consistent and knowledge-enhanced responses.

==> figures/data_sample_latex.tex <==
\begin{figure}[t]
\centering
\includegraphics[trim={0cm 1cm 0cm 1cm}, clip, scale=0.2, width=0.5\textwidth]{figures/data_sample.pdf}
%width=77.125mm
\captionsetup{font=10pt}
\caption{A sample from the KBP dataset. There are three situations of responses in our datasets: 1) response without the need for any sources (\texttt{NULL}), 2) response using only personae description (from \texttt{PERSONA} source), and 3) response using both persona and knowledge (from \texttt{PERSONA, DOCUMENTS} sources). The example here presents the first and third situations.}
\label{data_sample}
\end{figure}

==> figures/dependency_latex.tex <==
\begin{figure}[t]
\centering
\includegraphics[trim={5cm 4cm 6cm 3.5cm}, clip, scale=0.2, width=0.5\textwidth]{figures/dependency.pdf}
%width=77.125mm
\captionsetup{font=10pt}
\caption{Another example to illustrate the dependency between different sources}
\label{data_sample}
\end{figure}

==> figures/number.tex <==
\begin{figure}[t]
\centering
\includegraphics[trim={0.1cm 0.3cm 0cm 0cm}, clip, scale=1.0, width=0.5\textwidth]{figures/retriever_number.pdf}
%width=77.125mm
\captionsetup{font=10pt}
\caption{The performance of \textbf{Retrieval} and \textbf{Assembly} using different number of retrieved results. B-P and B-K stand for \texttt{PERSONA} and \texttt{KNOWLEDGE} in Both in Table~\ref{tab:retriever}}
\label{number_ana}
\end{figure}
